Towards Bounded Infeasible Code Detection

A first step towards more reliable software is to execute each statement and each control-flow path in a method once. In this paper, we present a formal method to automatically compute test cases for this purpose based on the idea of a bounded infeasible code detection. The method first unwinds all loops in a program finitely often and then encodes all feasible executions of the loop-free programs in a logical formula. Helper variables are introduced such that a theorem prover can reconstruct the control-flow path of a feasible execution from a satisfying valuation of this formula. Based on this formula, we present one algorithm that computes a feasible path cover and one algorithm that computes a feasible statement cover. We show that the algorithms are complete for loop-free programs and that they can be implemented efficiently. We further provide a sound algorithm to compute procedure summaries which makes the method scalable to larger programs.

==> Makefile <==
FNAME=main
TEXINPUTS= TEXINPUTS=./
BIBINPUTS= BIBINPUTS=./

BIBTEX=$(BIBINPUTS) bibtex
TEXDEPEND=$(TEXINPUTS) $(BIBINPUTS) texdepend -out .depend -format make -expand
#TEX=$(TEXINPUTS): latex -halt-on-error
#TEXEXT=dvi
TEX=$(TEXINPUTS): pdflatex -halt-on-error
TEXEXT=pdf
$(FNAME).pdf: data/c01.pdf \
	data/qall.pdf data/tall.pdf

all: $(FNAME).pdf

$(FNAME).$(TEXEXT): $(wildcard *.tex) $(wildcard *.sty) $(FNAME).bib
%.$(TEXEXT):  %.tex 
	$(TEX) $< && \
	$(BIBTEX) $(*F) && \
	$(TEX) $< && \
	$(TEX) $<

%.ps: %.dvi
	dvips -Ppdf $? -o $@

%.pdf: %.ps
	ps2pdf $?

%.pdf: %.eps
	epstopdf $<

depend:
	$(TEXDEPEND) $(FNAME).tex

-include .depend

$(FNAME).dvi: $(INCLUDES) $(FIGS) $(BIB_FILES) $(STYLES)

clean:
	rm -f *~ *.~ *.log *.aux *.toc *.bbl *.blg *.out \
	$(FNAME).dvi $(FNAME).ps


==> exvc.tex <==
%\section{Extended Weakest-Liberal Precondition}\label{sec:exvc}

That is, in a satisfying valuation of the VC, each block variable
$B_{\texttt{label\_i}}$ is assigned to $\true$ if, for any pre-state, there exists a terminating
execution starting in $\texttt{label\_i}$.

However, it is not enough to find one $\true$ evaluation for each 
$B_{\texttt{label\_i}}$ to cover the entire graph.
To efficiently find valuations which cover the whole CFG, we want to
have helper variables which are true if and only if there is a normal
terminating execution of that block starting in the initial state of the
program. If we have a satisfying valuation in which
$B_{\texttt{label\_i}}$ is set to $\true$, we only know that there is a normal
terminating execution starting at $B_{\texttt{label\_i}}$. It does not say that
this execution can be extended to one starting in the initial block.  

Even if we might find a valuation where  $B_{\texttt{label\_i}}$ is $\true$ it still
might be unreachable. Hence, to avoid encoding all paths simultaneously (and
thus adding redundancy again), we need helper variables:

We invert the directions of the edges in the CFG and for each block: 
$$\texttt{label} : S; \textbf{comefrom}
(\texttt{label\_1}\ldots\texttt{label\_n}) $$
we generate an auxiliary variable $R_{\texttt{label}}$ and a formula
$$
RTerm_\texttt{label} : R_{\texttt{label}} \equiv B_{\texttt{label}} \wedge
\bigvee_{1\leq i\leq n} R_{\texttt{label\_i}} ) 
$$

Our new verification condition looks as follows:
$$
EXVC := (\wedge_{i} RTerm_\texttt{label\_i}) \wedge (\wedge_{i}
Term_\texttt{label\_i}) \wedge  \neg B_{\texttt{label\_0}} 
$$

\begin{theorem}
Something like: Given $VC$ and $EXVC$. A valuation $\val$ satisfies $EXVC$ if
and only if $\val$ also satisfies $VC$ and for each $RTerm_\texttt{label}$ with
$\phi(RTerm_\texttt{label})=\true$ there exists a normal terminating execution
in the program.
\end{theorem}

Now, the problem of finding a set of valuations satisfying this formula
which already covers the entire CFG quickly corresponds to the problem of
finding a $\true$ valuation for all $RTerm_\texttt{label}$ as fast as possible.





